Chemistry-Inspired Pattern Formation with Robotic Swarms

Self-organized emergent patterns can be widely seen in particle interactions producing complex structures such as chemical elements and molecules. Inspired by these interactions, this work presents a novel stochastic approach that allows a swarm of heterogeneous robots to create emergent patterns in a completely decentralized fashion and relying only on local information. Our approach consists of modeling the swarm configuration as a dynamic Gibbs Random Field (GRF) and setting constraints on the neighborhood system inspired by chemistry rules that dictate binding polarity between particles. Using the GRF model, we determine velocities for each robot, resulting in behaviors that lead to the creation of patterns or shapes. Simulated experiments show the versatility of the approach in producing a variety of patterns, and experiments with a group of physical robots show the feasibility in potential applications.

==> sections/03_background.tex <==
\section{Background}
\label{sec:background}

% In this section, we overview some concepts about \textit{Gibbs Random Fields} (GRFs) explaining their properties and why they make sense in a swarm robotics context.
% A GRF is a probabilistic graphical model that is a particular case of the  \textit{Markov Random Field} (MRF) when the joint probability density of the random variables is strictly positive. GRF models are based on local interactions between neighboring agents. The Markov property is a conditional property that allows one to ignore more distant information as soon as local information is provided. The Hammersley-Clifford theorem establishes the equivalence between \rev{a} MRF and a GRF~\cite{kindermann1980markov}. %Here we are not going to demonstrate such equivalence, but only present an overview of a MRF towards a GRF.

% To describe these models succinctly, assume an undirected graph $\mathbf{G} = (\mathbf{V},\mathbf{E})$ with vertices as spatial sites and indexed by $v = 1, 2, . . . , \eta$. A random field on $\mathbf{G}$ is as collection of random variables $\mathbf{X} = \{X_{v}\}_{v \in \mathbf{V}}$ and, for each $v \in \mathbf{V}$, let $\Lambda_v$ be finite set called the phase space for site $v$ that represents where the random variable $X_v$ takes it values.
% % ≜ -> is equal by definition to  
% An instance of $\mathbf{X}$ establishes a state of the random field $x = \{(x_1,..., x_\eta): x_v \in \Lambda_v, v \in \mathbf{V}\}$ and the product space $\Lambda \triangleq \Lambda_1 \times ... \times \Lambda_\mathbf{\eta} $ forms the configuration space. 

% A neighborhood system on $\mathbf{V}$ is a family $\mathcal{N} = \{\mathcal{N}_v\}_{v \in \mathbf{V}}$, where $\mathcal{N}_v \subset \mathbf{V}$ is the set of neighbors for site $v$ satisfying $v/\mathcal{N}_v$ and $r \in \mathcal{N}_v \Leftrightarrow v \in \mathcal{N}_r$. 
% %
% The neighborhood system induces the configuration of the undirected graph $\mathbf{G}$ by setting 
% %with vertices $v, r \in \mathbf{V}$, and 
% an edge $\{v,r\} \in \mathbf{E}$ between $v$ and $r$ if and only if $r \in \mathcal{N}_v$. A set $\mathcal{C} \subset \mathbf{V}$ is called a \textit{clique} if all elements of $\mathcal{C}$ are neighbors of each other. 

% Thus, a random field $\mathbf{X}$ is called an MRF concerning the neighborhood system $\mathcal{N}$ if, $\forall v \in \mathbf{V}$,
% \begin{equation}
% \displaystyle{
%     P(X_v=x_v \text{$|$} (X_r=x_r)_{r \neq v}) = P (X_v=x_v \text{$|$} (X_r=x_r)_{r \in \mathcal{N}_v})},
% \label{eq:mrf}
% \end{equation}
% %where $\displaystyle{P(\cdot|\cdot)}$ denotes the conditional probability of the event $e_1$ given that the event $e_2$ happens. 
% which indicates that the probability of the site $v$ assuming the state $x_v$ given the state of all other sites is equal to the probability of $v$ assuming the same state $x_v$ given only the states of neighboring sites. Such a definition reflects the local characteristics of the MRF constrained by the local Markov properties~\cite{koller2009probabilistic}\rev{. It is} convenient to model robotics swarms, since it implies the conditional independence of information coming from outside a neighborhood system, which supports the requirement of local interactions. 

% %A remark for (\ref{eq:mrf}) is that it reflects the local characteristics of the MRF constrained by the local Markov properties~\cite{koller2009probabilistic}. Such constraints may be convenient to model swarm robots since it implies the independence of information coming from outside a neighborhood system, which supports the requirement of local interaction. 

% % By definition, an MRF satisfies the following Markov properties:  
% %  \subsubsection{Pairwise Markov property} Any two non-neighbors variables are conditionally independent given all other variables: 
% %  \begin{align*}
% %      X_{u} \perp \!\!\!\perp X_{v} \mid X_{V \setminus \{u,v\}}.
% %  \end{align*}

% % \subsubsection{Local Markov property} A variable is conditionally independent of all other variables given its neighbors:
% % \begin{align*}
% %  X_{v}\perp \!\!\!\perp X_{V\setminus \mathcal{N}_{v+}}\mid X_{\mathcal{N}_v},
% %  \end{align*}
% % where $\mathcal{N}_v$ is the set of neighbors of $v$, and $\mathcal{N}_{v+}=v\cup \mathcal{N}_v$ is the closed neighborhood of $v$.

% % \subsubsection{Global Markov property} Any two subsets of variables are conditionally independent given a separating subset:
% %     \begin{align*}
% %     X_{A}\perp \!\!\!\perp X_{B}\mid X_{S},
% %     \end{align*}
% % where a separating subset $S$ is one in which every path from a subset $A$ to a subset $B$ passes through it.
% %
% % In general, the last property is stronger than the second one, which in turn is stronger than the first one. But, if the probability is positive, the above three Markov properties are equivalent~\cite{koller2009probabilistic}. 
% %Such constraints may be convenient to model swarm robots since it implies the independence of information coming from outside a neighborhood system, which supports the requirement of local interaction. 

% %A GRF is a particular application for (\ref{eq:mrf}) when its joint probability density can be represented by the Gibbs measure. 
% \rev{A GRF is a particular application for (\ref{eq:mrf}) when the Gibbs measure can represent its joint probability density.} A Gibbs measure is a generalization of the canonical ensemble to infinite systems, which gives the probability of the system $\mathbf{X}$ being in the state $x$. Formally, let us denote a potential $\mathbf{U}$ as a family $\displaystyle{\{U_A : A \subset \mathbf{V}\}}$ of functions on the configuration space $\Lambda$, where $U_A : \Lambda \rightarrow \mathbb{R}$, and $U_A(x)$ depends only on $x_A \triangleq \{x_v: v \in A\}$. At the end, $U_A$ is only a function of the values at the sites contained in the set $A$, that is $\displaystyle{U_A(x) \equiv U_A(x_A)}$. In this way, given a potential $\mathbf{U}$, the potential energy $H(x)$ for configuration $x$ is defined as
% \begin{equation}
% H(x) = \sum \limits_{A \subset \mathbf{V}} U_A(x_A).
% \label{eq:potentialenergy1}
% \end{equation}

% By definition~\cite{kindermann1980markov}, if $U_A \equiv 0$ whenever $A$ is not a \textit{clique} or a singleton, $\mathbf{U}$ is called a nearest-neighbor potential. If $U_A \equiv 0$ whenever $A$ is not a pair or a singleton, $\mathbf{U}$ is called a pairwise potential. $\mathbf{U}$ is called a pairwise, nearest-neighbor potential if it is both a pairwise potential and a nearest-neighbor potential. In particular, for a pairwise, nearest-neighbor potential $U$, we can write (\ref{eq:potentialenergy1}) as
% \begin{equation}
% H(x) = \sum \limits_{v \in \mathbf{V}} U_{\{v\}}(x_v) + \sum \limits_{(v,t) \in \mathbf{V}  \times \mathbf{V}, t \in \mathcal{N}_v} U_{\{v,t\}}(x_v, x_t).
% \label{eq:potentialenergy2}
% \end{equation}

% Finally, a random field $\mathbf{X}$ is called a GRF if,
% \begin{equation}
%     P(\mathbf{X} = x) = \frac{1}{Z}e^{-\frac{H(x)}{T}}, \textrm{ with } Z = \sum \limits_{z} e^{-\frac{H(z)}{T}},
%     \label{eq:gibbsdistribution}
% \end{equation}
% where $Z$ is the partition function (normalizing constant); $T$ is interpreted as temperature in the context of statistical physics; and $\frac{1}{Z}e^{-\frac{H(x)}{T}}$ is called Gibbs distribution. 
% %A remark for (\ref{eq:gibbsdistribution}) is that a higher-energy state implies a lower probability and that the influence of energy on probability increases as $T$ decreases. 

% Researchers in statistical mechanics and mathematics usually applied the GRF to describe the distribution of system configurations at the thermodynamic equilibrium or measure the probability of such a system \rev{yielding} the desired state. One of the challenges of directly evaluating~(\ref{eq:gibbsdistribution}) is the high cardinality of the configuration space, which makes the computation of $Z$ intractable.

% A typical approach to sequential sampling states in a configuration space given a probability function consists of using Markov Chain Monte Carlo (MCMC) methods, such as the Metropolis algorithm~\cite{hastings1970monte}. A process to \rev{parallelly} sample over~(\ref{eq:gibbsdistribution}) is described in the next section.







==> sections/temp.tex <==
\subsection{Applications} % or Other behaviors
As we state,  the combination of segregative and flocking behaviors allows the execution of several complex tasks. Further, we intend to deal with such tasks using the methodology presented in this work. For instance, we aim to investigate swarm transportation and shape-formation in the context of heterogeneity groups. Fig.~\ref{fig:segregationexp} shows an initial step toward to shape-formation. 

\begin{figure}[h]
	\begin{subfigure}{.18\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{figures/verlab/img0001.png}
		\caption{$n=0$}
		\label{fig:rangerobots}
	\end{subfigure}%
    \hspace*{-1.2em}
	\begin{subfigure}{.18\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{figures/verlab/img0042.png}
		\caption{$n=200$}
		\label{fig:rangegroups}
	\end{subfigure}%
    \hspace*{-1.2em}
	\begin{subfigure}{.18\textwidth}
		\centering
		\includegraphics[width=.95\linewidth]{figures/verlab/img0322.png}
		\caption{$n=1600$}
		\label{fig:shapeformation}
	\end{subfigure}%
	\caption{Initial steps toward shape-formation task. Virtual points with heterogeneous attraction are placed in the environment so that robots of a specific type are attracted, resulting in the formation of structures. A video is available at \url{https://youtu.be/uJs0fwiQHIc}.} % footnote
	\label{fig:segregationexp}
\end{figure}



\begin{algorithm}[t]
\caption{Calculate robot $i$ velocity at time $t+1$}\label{alg:metropolis}
\Procedure{Update}{$\mathbf{q_i}^{(t)}, \mathbf{v_i}^{(t)}$} 
 \State $\mathbf{V}^{(0)} \gets \mathbf{v_i}^{(t)}$, \Comment{Set of velocities} 
 \State $\mathbf{U}^{(0)} \gets H(\mathbf{q_i}^{(t)}, \mathbf{v_i}^{(t)})$, \Comment{Set of potential energies} 
 \For{$k \gets 1$ to $\mathcal{I}$}
%  \State $\mathbf{v}_{prev} \gets \mathbf{V}$(end),  \Comment{Get the last element of $\mathbf{V}$} 
%  \State $\mathbf{u}_{prev} \gets \mathbf{U}$(end),  \Comment{Get the last element of $\mathbf{U}$} 
 \State $\bar{\mathbf{v}} \gets N(\mathbf{v_i}^{(t)}, \mathbf{\Sigma})$,    \Comment{Gaussian sampling} 
 \State $\bar{\mathbf{u}} \gets  H(\mathbf{q_i}^{(t)}, \bar{\mathbf{v}})$,
 \State $\Delta E \gets \bar{\mathbf{u}} - \mathbf{U}^{(k-1)}$,      \Comment{Potential energy variation}
 \State $g \gets exp(-\Delta E)$,   \Comment{Compute the gibbs energy}
 \State $r \gets \mathcal{U}(0, 1)$,   \Comment{Uniform sampling}
 \If{$(\Delta E < 0) \lor (r < g)$ } \Comment{Sample is accepted}
    \State $\mathbf{V}^{(k)} \gets \bar{\mathbf{v}}$,
    \State $\mathbf{U}^{(k)} \gets \bar{\mathbf{u}}$,
    \Else \Comment{Sample is rejected}
    \State $\mathbf{V}^{(k)} \gets  {\mathbf{V}^{(k-1)}}$,
    \State $\mathbf{U}^{(k)} \gets  {\mathbf{U}^{(k-1)}}$,
    \EndIf
 \EndFor
%  \State $\mathbf{V} \gets \mathbf{V}^{(j,...,\mathcal{I})}$, \Comment{Reject the first j velocities}
 \State $\mathbf{v_i}^{(t+1)} \gets  (\mathbf{V}^q + ...+\mathbf{V}^\mathcal{I})/(\mathcal{I}-q)$, \Comment{Average velocity}
 \State \textbf{return} $\mathbf{v_i}^{(t+1)}$
\EndProcedure
\end{algorithm}


% \subsection{Formation of complex patterns}
% A well-known mechanism to generate patterns of interest maintaining locality assumptions consists of using robots as anchors. These robots are placed in specific positions of the environment to induce the convergence of the rest of the swarm in that pattern.

% Here %In this experiment, 
% we set up a specific type of robot and place it in points of the patterns. The interaction of these robots with others follows the same rules. 
% % However, they do not move and also do not coordinate the others. 
% In the first experiment, we investigated the swarm's ability to form the shape of a square. We placed nine anchor robots in the environment to form a square, and we uniformly spread a swarm of carbon-like and hydrogen-like robots. Figure~\ref{fig:pattern_square} shows that after a few iterations, the swarm was able to form structures resembling methane, and these were arranged in the shape of a square.

% In the second experiment, we varied the shapes of interest to form letters and used different combinations of robot types. Figure~\ref{fig:pattern_verlab} shows the swarm converging in the shape of the letters. An advantage of using robots as anchors to induce shapes is its simplicity and accuracy. Note that the last two letters are composed of three types of robots that form structures resembling molecules of water, methane, and ammonia, and each structure is bond with different types of anchor robots.


% The previous results show that one may define different binding constraints allowing the swarm to emerge with various patterns. However, it is not straightforward to define rules that generate specific forms due to the system's dynamic. However, if we assume the use of typical mechanisms from literature, we can induce the swarm to produce more complex shapes. By placing seed robots in the environment to define a shape, we can induce the rest of the swarm to form it.

% This experiment shows that our method can be extended to use typical pattern formation mechanisms. In addition, we also demonstrate its performance in a realistic, physics-based simulated environment set up in the Gazebo simulator. We use ROS middleware to implement our method, demonstrating the robustness against noise in sensors and actuators and the decentralized processing capacity. The figure shows the results of this experiment. A video is available at Youtube~\footnote{\url{https://youtu.be/liTdCWZMevc}}.

% V-letter = https://youtu.be/0Wm7eFIZ_FI
% E-letter = https://youtu.be/k_20CHdjLIU
% R-letter = https://youtu.be/N1vOIOyzWQQ
% L-letter = https://youtu.be/XAjzLcWOhkM
% A-letter = https://youtu.be/xDe0VwngSCs
% B-letter = https://youtu.be/o_pvequKnkk

% As shown above, the pattern formation depends on how some constraints are defined. As patterns emerge from these rules, it is not trivial to define rules that generate specific forms. However, if we assume the use of typical mechanisms in the form formation literature, we can induce the swarm to form shapes. One such mechanism is to place seed in the environment where the robots should be. These points have a specific shape. By assuming these virtual robots as anchors and assert bond restrictions, we can induce the swarm to attract to these anchors, forming the pattern. The figure shows the results of this experiment.

% \begin{figure*}[t] % <---------------------------------- VERLAB
% 	\begin{subfigure}{.99\textwidth}
% 		\centering
% 		\includegraphics[width=.99\linewidth]{images/pattern_square.pdf}
% 		\caption{}
% 		\label{fig:pattern_square}
% 	\end{subfigure}
% 	\qquad
% % 	\hspace*{-1.4em}
% 	\begin{subfigure}{.99\textwidth}
% 		\centering
% 		\includegraphics[width=.99\linewidth]{images/pattern_verlab.pdf}
% 		\caption{}
% 		\label{fig:pattern_verlab}
% 	\end{subfigure}
% 	\caption{Simulations showing the formation of patterns of interest: (a) snapshot sequence showing the formation of a square, and (b) the formation of letters: VERLAB.}
% 	\label{fig:pattern_snapshots}
% \end{figure*}





% To evaluate the performance of our approach, we conduct a series of simulated experiments. We first analyze the segregative behavior by measuring the \rev{method's performance} %performance of the method 
% for different configurations and comparing the results with other methods from the literature. Then, to analyze the flocking capabilities, we evaluate the velocity consensus \rev{and} %as well as 
% the cohesion among the robots when there is noise in the sensor. Finally, we performed experiments with real robots as a proof-of-concept to show the feasibility of our approach in real scenarios. 
% %and present other behaviors that we further intend to study. 
% Fig.~\ref{fig:snapshots} shows snapshots illustrating the simultaneous flocking segregative behavior produced by our methodology. A video of the experiments is available at Youtube\footnote{\url{https://youtu.be/KooNGIStWlM}} and the source code at Github\footnote{\url{https://github.com/verlab/2021-icra-grf-swarm}}.


% \subsection{Segregation Analysis}
% To evaluate the segregative behavior considering only local information, we compare the convergence rate of our approach against the one presented by Mitrano et al.~\cite{mitrano2019minimalistic} and Inácio et al.~\cite{inacio2019pso}. We consider the work proposed by Santos et al.~\cite{santos2020spatial} as a baseline since it assumes global knowledge about the positions of other robots leading to a fast convergence rate. We also contrast our methodology with a deterministic gradient descent approach using potential differentials to show that such mechanism may be easily trapped at local minima.

% The experiments consisted of $100$ runs of each approach with a maximum of $20000$ iterations. \rev{A random initial state is generated for each run, but it is the same for all approaches.} %For each run, a random initial state is generated, but it is the same for all approaches. 
% At each iteration, the robot \rev{can} move a maximum of $0.02$ meters in a square area of $10$ by $10$ meters with the walls being considered obstacles. We varied the number of robots and the number of heterogeneous groups
% %, and the sensing distance 
% to evaluate each \rev{approach's performance.} %the performance of each approach. 
% As a metric, we compute the total amount of clusters formed by robots of the same type \rev{and} %as well as 
% the number of iterations necessary to reach it. Here, two robots of the same type are considered to be in the same cluster if their relative distance is less than $0.3$ meters -- the robot radius is $0.07$ meters. The sensing range is set to $0.5$ meters ($\lambda=0.5$) Fig.~\ref{fig:segregationexp} shows the mean and the $99\%$ confidence interval comparing one with the other approaches.

% \begin{figure}[h]
% 	\begin{subfigure}{.465\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/exp_seg_1.eps}
% 		\caption{}
% 		\label{fig:rangerobots}
% 	\end{subfigure}%
% 	\qquad
% 	\begin{subfigure}{.465\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/exp_seg_2.eps}
% 		\caption{}
% 		\label{fig:rangegroups}
% 	\end{subfigure}%
% %	\qquad
% %	\begin{subfigure}{.47\textwidth}
% %		\centering
% %		\includegraphics[width=.95\linewidth]{figures/exp_seg_3.eps}
% %		\caption{}
% %		\label{fig:rangesensing}
% %	\end{subfigure}%
% 	\caption{The minimum number of clusters yield by each approach in up to $20000$ iterations when: (a) we increase the number of robots $|\tau_m| = \{10,30,60\}$ keeping $|\tau|=5$ heterogeneous groups; and (b) we increase the number of groups $|\tau|=\{5, 15, 30\}$ keeping $|\tau_m| = 10$ robots per group.
% 	% and sensing range $\lambda=0.5$ meters.
% 	%; and (c) increases the sensing range $\lambda =\{0.5, 1.5, 3.0\}$ keeping  $|\tau_m| = 30$ robots and $|\tau|=5$ heterogeneous groups.
% 	} % footnote
% 	\label{fig:segregationexp}
% \end{figure}

% %In general, our approach remained competitive with the strategy presented by Inácio et al.~\cite{inacio2019pso}, obtaining better results while the second was faster. Increasing the sensing range, we observe that our approach overcomes Inácio's method regarding number of iterations, since it behaves worse due to the congestion problem. The minimalist approach proposed by Mitrano et al.~\cite{mitrano2019minimalistic} presents interesting results in several situations but is in general slower. Regarding the advantage of using a stochastic approach over a gradient descent-type algorithm, we observe that such a mechanism is easily trapped to a minimum of potential, preventing it from converging to better results in comparison to our potential functions.

% Analyzing the segregation using the number of formed clusters, we can see that all approaches executed relatively well for a small number of groups, even for an increasing number of robots per group (Fig. \ref{fig:rangerobots}, top). \rev{The exception is the Gradient-Descent method, which gets trapped in local minima and cannot reach a segregated state.} %The exception is the Gradient-Descent method, that gets trapped in local minima and is not able to reach a segregated state. 
% When the number of groups increases, our approach significantly outperforms the others, with a performance close to the baseline which uses global information (Fig. \ref{fig:rangegroups}, top). When there is a large number of groups, robots usually get trapped by other groups and cannot reach a segregated state. By relying on the stochastic nature of the GRF, our approach \rev{can handle these situations better.} %is able to better handle these situations. 
% %---- Esse restante sai se tirarmos a figura (c)
% %When we increase the sensing range, our method continues to execute well while the others degrade a little (Figure \ref{fig:rangesensing}). While our method takes advantage of a larger sensing area to ``capture'' more robots and converge faster, other methods, specially Inacio et al. that rely on communication among neighboors, can have problems to reach consensus.

% Regarding the performance in terms of \rev{the} number of iterations to reach segregation, we can see that the methods have a similar performance \rev{on} average when increasing the number of robots. \rev{However, all} of them are significantly slower than the baseline, which uses global information (Fig. \ref{fig:rangerobots}, bottom). When we vary the number of groups, we can see that Inácio et al. \rev{have} a better performance (Fig. \ref{fig:rangegroups}, bottom). However there may be a caveat, specially for $|\tau| = 30$: our metric considers the number of iterations spent until reaching the minimum number of clusters. As previously mentioned, Inácio's method does not reach the minimum number of clusters \rev{on} several occasions. So, it may be converging faster but to a sub-optimal configuration. \rev{On the other hand, our method may take} %Our method, on the other hand, may take
% longer due to its stochastic nature, but has a much better success rate. 
% %---- Esse restante sai se tirarmos a figura (c)
% %Finally, our method performs better in comparisson to the others when we increase the sensing range for the same reasons mentioned in the cluster analysis.


% \subsection{Flocking Analysis}
% To evaluate the effectiveness of our approach in producing flocking behaviors, we carried out some experiments and \rev{analyzed} them regarding the average distance (cohesion) and consensus speed between robots of the same type. The robustness of our method is assessed by adding Gaussian noise $\epsilon$ to the sensor model so that the relative position and velocity estimates are not reliable. Here, we perform $100$ runs with a maximum of $20000$ iterations. We assume $|\tau_m| = 30$ robots into $|\tau|=5$ heterogeneous groups and sensing range $\lambda=0.5$ meters. The robots start each run in a random initial state and perform both segregation and flocking within an environment of 10 by 10 meters at a maximum speed of $v_{max}=1.0$ meters per second. Noise in the sensor model ranges from $\epsilon = \{0\%, 2\%, 6\%, 10\%\}$ for both relative position and velocity. A noise of $\epsilon = 10\%$ implies an error of up to $10\%\lambda = 0.05$ meters in position and $10\%v_{max} = 0.10$ meters per seconds in speed. Fig.~\ref{fig:navigation} shows the mean and the $95\%$ confidence interval evaluating the impact that such a noise causes in our methodology.

% As expected, increasing noise in the sensor model significantly impacts the velocity consensus. We observed that up to $\epsilon = 6\%$, the swarm is able to maintain the flocking-segregative behavior for the \rev{experiments' configuration}. %configuration of the experiments. 
% When $\epsilon = 10\%$, we notice the velocity consensus degrading and, consequently, the flocking behavior does not converge. However, even with \rev{the} noise we \rev{can} %are able to 
% segregate the swarm to the minimal number of clusters most of the times for a sufficiently large number of iterations.

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=.87\linewidth]{figures/exp_nav.eps}
% 	\caption{Impact of the noise in the sensor model \rev{on} the performance of our method. The graphics display the number of clusters yield, the average distance, and velocity error among \rev{the same group of robots} in up to $20000$ iterations.}
% 	%A video is available at \url{https://youtu.be/okdSnqL4Q3k}.}
% 	\label{fig:navigation}
% \end{figure}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Real Experiments
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Real robots}
% To evaluate the feasibility of our approach in a real environment, we performed proof-of-concept experiments using five e-puck robots~\cite{mondada2009puck}. The robots receive velocity commands from a remote server executing ROS. Given that our robots do not have any sensor that allows them to estimate the relative position and velocity of neighboring robots, we emulate such a sensor using the Optitrack motion capture system~\cite{optitrack}.

% Here we consider the bounded environment as a square area of 2 by 2 meters restricted by walls. We set the sensing distance to $\lambda = 0.3$, and as we have only a few robots, we evaluate cases where we have one or two groups. That is one group with five robots and two groups with two and three robots each. Fig.~\ref{fig:realplot} shows the performance of our approach using real robots. We can see that the robots can reach segregation and also keep the flocking behavior, but with some noise in the velocity consensus due to the uncertainties observed in real settings. 

% \begin{figure}[h]
% 	\centering
% 	\includegraphics[width=.87\linewidth]{figures/2020-10-13-14-53-06.eps}
% 	\caption{Results on real experiments using five epuck robots divided into one or two groups. }
% 	%A video is available at \url{https://youtu.be/_ls5IkB7zNE}.}
% 	\label{fig:realplot}
% \end{figure}

% % \begin{figure}[h]
% % 	\begin{subfigure}{.16\textwidth}
% % 		\centering
% % 		\includegraphics[width=.95\linewidth]{figures/real/img000001}
% % 		\caption{$n=0$}
% % % 		\label{fig:rangerobots}
% % 	\end{subfigure}%
% %     \hspace*{-0.5em}
% % 	\begin{subfigure}{.16\textwidth}
% % 		\centering
% % 		\includegraphics[width=.95\linewidth]{figures/real/img000244}
% % 		\caption{$n=244$}
% % % 		\label{fig:rangegroups}
% % 	\end{subfigure}%
% %     \hspace*{-0.5em}
% % 	\begin{subfigure}{.16\textwidth}
% % 		\centering
% % 		\includegraphics[width=.95\linewidth]{figures/real/img000426}
% % 		\caption{$n=426$}
% % % 		\label{fig:shapeformation}
% % 	\end{subfigure}%
% % 	\caption{$8$ robots segregating into $2$ heterogeneous groups and navigating within a $2$ by $2$ meters environment. A video is available at \url{https://youtu.be/DzGWStU99dI}.} % footnote
% % 	\label{fig:grfreal}
% % \end{figure}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% % Applications
% %%%%%%%%%%%%%%%%%%%%%%%%%%%
% % movi para o temp.tex




















% \subsection{}
% \subsection{What should be evaluated?}
% \begin{itemize}
%     \item Potential between two robots (same type; different type)
%     \item Average Distance between groups and robots same type
%     \item Segregation Metrics per time with confidence interval
%     \item Noise sensor and actuation
%     \item Comparison with VGS and Tan
% \end{itemize}

% \subsection{Videos}
% \subsubsection{Dense Environment with Multi Groups}
% \subsubsection{Dense Environment with few groups}
% \subsubsection{Sparse Environment with few groups}

%\begin{figure}
	%\begin{subfigure}{.4\textwidth}
		%\centering
		%\includegraphics[width=.90\linewidth]{figures/sim}
	%\end{subfigure}
	%\caption{Collective swarm mapping in simulated environment. The blue squares represents the robots, while the large blue circles represents the sensor range.} 
	%\label{fig:stage}
%\end{figure}


%\begin{figure}
%		\centering
%		\includegraphics[width=.60\linewidth]{figures/sim}
%	\caption{Swarm mapping in a simulated environment with 2 obstacles. The blue squares represent the robots, while the gray circles around them represent the sensor range.} 
%	\label{fig:stage}
%\end{figure}

% Specifically, as will be presented in the next sections, we analyze the impacts of the localization errors and swarm size in the map quality using different simulated scenarios. Moreover, we performed proof of concept experiments using a team of 9 e-puck robots to show the efficacy of the methodology in real scenarios.

% \subsection{Simulated Experiments}

% For the simulations, robots were programmed using the Robot Operating System (ROS)
% %~\cite{quigley2009ros} 
% and executed in the Stage Simulator.
% %~\cite{gerkey2003player}. 
% We used simple differential kinematic robots equipped with low range exteroceptive sensors. 
% %Figure~\ref{fig:stage} shows a snapshot of these experiments on the Stage simulator. 
% All localization estimation, obstacle avoidance, neighborhood perception and motion control calculations were processed individually by each robot node on ROS, and the pair-to-pair communication were emulated between each node using ROS services. The map is computed in a different ROS node implemented as an independent process. All the robots publish their pose and sensing information to a ROS topic that is listened by the map node. As mentioned, the occupancy grid updates are computed as soon as new information is received, ordered by a buffer queue. 

% To simulate localization errors, we considered the motion model presented in \cite{thrun2005probabilistic}, with noise parameters $\mathbf{\alpha_\epsilon} = [0.05, 0.05, 0.05, 0.05]$. These were empirically determined to be close to the errors obtained in real experiments. We used a robot range perception and communication radius of $1m$ and each robot can achieve a maximum velocity of $1m/s$. The range sensor uses an ultrasonic model, with resolution of 22.5 degrees (16 sensors).

% Our first experiment evaluates the quality of the occupancy grid maps generated by SwarMap. We performed the task using 36 robots in a $16\times16m$ squared environment with 2 obstacles. The robots explored the environment for 300 seconds. We performed several runs with this setup, and Figure~\ref{fig:rr} shows the occupancy grid maps generated on a typical run. The maps generated by the SwarMap (Figure~\ref{fig:rr}(c) without a GPS robot and Figure~\ref{fig:rr}(d) with a GPS robot) are compared with an occupancy grid generated with perfect localization, which we refer as ground truth (Figure~\ref{fig:rr}(a)), and with an occupancy grid generated by robots that localize through dead reckoning only, without any information exchange between agents (Figure~\ref{fig:rr}(b)).  

% \begin{figure}[t]
% 	\begin{subfigure}{.23\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/real/gt_36_300}
% 		\caption{Ground Truth}
% 		\label{fig:rr1}
% 	\end{subfigure}%
% 	\begin{subfigure}{.23\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/real/odom_36_300}
% 		\caption{Only Odometry}
% 		\label{fig:rr2}
% 	\end{subfigure}
% 	\begin{subfigure}{.23\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/real/filtered_36_300}
% 		\caption{SwarMap without GPS}
% 		\label{fig:rr3}
% 	\end{subfigure}
% 	\begin{subfigure}{.23\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/real/filtered_gps_36_300}
% 		\caption{SwarMap with 1 GPS}
% 		\label{fig:rr4}
% 	\end{subfigure}
% 	\caption{Maps generated in simulations with 36 robots exploring an  environment during $300$ seconds.} 
% 	%Figure \ref{fig:rr1} is the resulting map considering that all robots have perfect estimation of their pose. Figure \ref{fig:rr2} is the result considering only individual odometry measurements and no data sharing between robots. Figure \ref{fig:rr3} shows the results for SwarMap algorithm without global localization and \ref{fig:rr4} considers the same algorithm with one agent in the swarm equipped with a GPS.} 
% 	\label{fig:rr}
% \end{figure}

% \begin{figure*}[t]
% 	\centering
% 	\begin{subfigure}{0.25\textwidth}
% 		\centering
% 		\includegraphics[width=.95\textwidth]{figures/map2/filtered_12_010_t-300}
% 		\caption{12 robots}
% 		\label{fig:res:map2-12}
% 	\end{subfigure}
% 	\begin{subfigure}{0.25\textwidth}
% 		\centering		
%         \includegraphics[width=.95\textwidth]{figures/map2/filtered_24_010_t-300}
% 		\caption{24 robots}
% 		\label{fig:res:map2-24}
% 	\end{subfigure}
% 	\begin{subfigure}{0.25\textwidth}
% 		\centering
% 		\includegraphics[width=.95\textwidth]{figures/map2/filtered_36_010_t-300}
% 		\caption{36 robots}
% 		\label{fig:res:map2-36}
% 	\end{subfigure}
% 	\caption{Maps generated after $t=300s$ of exploration using (a) 12, (b) 24, and (c) 36 robots with one GPS per swarm.}
% 	\label{fig:res:map2}
% \end{figure*}


% As expected, the map quality is directly related to the localization accuracy. Combining data from different robots, the SwarMap significantly enhances the quality of the map in comparison to the approach that does not share information for localization. Moreover, the use of a single robot with absolute localization greatly improves the map quality. This can be observed comparing maps (c) and (d) of Figure \ref{fig:rr}. It is interesting to note that this improvement is not restricted to specific regions, suggesting that the accurate pose estimates from the robot with the GPS are spread in a multi-hop fashion throughout the swarm.



% %Figure \ref{fig:rr} shows the resulting occupancy maps in an environment with two central obstacles explored by 36 robots. In this experiment, we compared our approach with the ground truth and the naive multi-robot pose estimation though dead recondition localization without any information exchange between agents. Comparing the results, it is possible to verify that the proposed mapping method is able to combine the information between agents, producing a better metric representation of the environment, even using only odometry information.   

% Another way of investigating the importance of information sharing among the swarm is to compare the map quality as we increase the number of robots in the swarm.  Figure~\ref{fig:res:map2} shows three maps generated by swarms of 12, 24 and 36 robots respectively. All of them have one robot with an absolute localization sensor. It is possible to observe that the map quality improves as the swarm size increases. With more robots in the swarm, the number of ``encounters" among robots will increase, boosting the share of information. This is very important, specially considering that we have robots with better estimates in the group.   

% This fact can be better observed evaluating the mean localization error over time for different sizes of swarms. Figure \ref{fig:perror} shows the localization Root Mean Square Error (RMSE) for a mapping task using homogeneous swarms of 12, 24 and 36 robots, and also using a swarm of 36 robots containing one agent with absolute localization. 

% It is easy to see that as the number of agents  increases, the average error of the group decreases, corroborating the idea that increasing the robot swarm size reduces significantly the swarm uncertainty and generate a better map. Furthermore, the placement of a GPS sensor in only one agent is enough to avoid the average error to diverge. 
% But we could not generalize these results to very large swarms, since with an increased density, robot to robot interference can start to take place, degrading the mapping results.

% %\begin{figure}
% %	\begin{subfigure}{.45\textwidth}
% %		\centering
% %		\includegraphics[width=\linewidth]{figures/rmse_mac.pdf}
% %		\caption{Position error}
% %		\label{fig:perror1}
% %	\end{subfigure}
% %	\begin{subfigure}{.45\textwidth}
% %		\centering
% %		\includegraphics[width=\linewidth]{figures/rmse_ang_mac.pdf}
% %		\caption{Orientation error}
% %		\label{fig:perror2}
% %	\end{subfigure}
% %	\caption{Average robot error estimation of pose while varying the number of robots on the same simulated environment.}
% %	\label{fig:perror}
% %\end{figure}

% \begin{figure}
% 		\centering		\includegraphics[width=0.94\columnwidth]{figures/rmse_mac}
% 	\caption{Average localization error estimation while varying the number of robots on the same simulated environment.}
% 	\label{fig:perror}
% \end{figure}




% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




% %\begin{figure}
% 	%\begin{subfigure}{.4\textwidth}
% 		%\centering
% 		%\includegraphics[width=.95\linewidth]{figures/expreal/path_error.pdf}
% 	%\end{subfigure}
% 	%\caption{Difference between pose estimation using GPS and odometry on an e-puck robot after 5 seconds of walk.} 
% 	%\label{fig:real_path}
% %\end{figure}
% %

% \subsection{Real Experiments}

% To evaluate the feasibility of our approach in a real environment,  we conducted proof-of-concept experiments using nine \textit{e-puck} robots. The \textit{e-puck}~\cite{mondada2009puck} is a small sized, differential wheeled platform equipped with a ring of eight infrared sensors, distributed with varied resolution (30° at the front, 45° at the sides and 60° at the back), capable of detecting objects within a $7.5$ centimeter range. It has a \textit{Bluetooth} interface that allows communication with a remote computer. In this remote computer, we use the \textit{ROS} framework for controlling the robot motion and also building the map in a similar way as done in the simulations.


% \begin{figure}
% \begin{center}
    
% 	\begin{subfigure}{.22\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/expreal/real_swarm_config_start.jpg}
% 		\caption{}
% 	    \label{fig:real_ex_a}
% 	\end{subfigure}%
% 	\begin{subfigure}{.22\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/expreal/real_swarm_config_middle_obs.jpg}
% 		\caption{}
% 	    \label{fig:real_ex_b}
% 	\end{subfigure}
% 	\caption{Example of a real experiment setup using nine e-pucks in two scenarios: (a) without obstacles and (b) with an obstacle in the center of the arena.} 
% 	\label{fig:real_ex}
% \end{center}

% \end{figure}

% Robots are also equipped with encoders that allow pose estimation through odometry. Besides the odometric information, an overhead camera system and a set of fiduciary markers were used for estimating the pose of each robot, providing global localization used as ground truth and GPS reference for evaluation. Also, since the robots are not equipped with bearing sensors, the overhead camera was used to provide the neighbors pose estimation $m^{ij}$, with a 10\% independent Gaussian noise added. 

% The real experiments were performed in an arena of about $1.85\times1.50m$ in our lab. Figure \ref{fig:real_ex_a} shows the robots before the start of an experiment in an environment without obstacles, while Figure \ref{fig:real_ex_b} shows the robots during exploration on a different  environment.

% The obtained results were in line with the simulations. Figure~\ref{fig:real_ex_rez} shows the maps produced by the real swarm after 200 seconds of exploration in a scenario with a single obstacle in the center of the arena. We can observe that the SwarMap algorithm using one GPS robot (Figure~\ref{fig:real_ex_rez}(d)) is capable of generating a reasonable map, compared with the ground truth (Figure~\ref{fig:real_ex_rez}(a)). On the other hand, the SwarMap without the GPS robot does not provide very good results. The main reason for that is the poor estimates obtained by the e-puck odometry, specially when the robots collide (due to failures in collision avoidance based on infrared), and the wheels slip on the floor. 

% \begin{figure}
% %	\begin{subfigure}{.24\textwidth}
% %		\centering
% %		\includegraphics[width=.95\linewidth]{figures/gt_001_t-200}
% %		\caption{Ground Truth}
% %	\end{subfigure}%
% 	\begin{subfigure}{.24\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/gt_001_t-203}
% 		\caption{Ground Truth}
% 	\end{subfigure}	
% %	\begin{subfigure}{.24\textwidth}
% %		\centering
% %		\includegraphics[width=.95\linewidth]{figures/odom_001_t-200}
% %		\caption{Odometry Only}
% %	\end{subfigure}%
% 	\begin{subfigure}{.24\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/odom_001_t-203}
% 		\caption{Odometry only}
% 	\end{subfigure}
% %	\begin{subfigure}{.24\textwidth}
% %		\centering
% %		\includegraphics[width=.95\linewidth]{figures/gfiltered_001_t-200}
% %		\caption{SwarMap}
% %	\end{subfigure}%
% 	\begin{subfigure}{.24\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/gfiltered_001_t-203}
% 		\caption{SwarMap}
% 	\end{subfigure}
% %	\begin{subfigure}{.24\textwidth}
% %		\centering
% %		\includegraphics[width=.95\linewidth]{figures/gfiltered_001_t-200_1}
% %		\caption{SwarMap + 1 GPS}
% %	\end{subfigure}%
% 	\begin{subfigure}{.24\textwidth}
% 		\centering
% 		\includegraphics[width=.95\linewidth]{figures/gfiltered_001_t-203_}
% 		\caption{SwarMap + 1 GPS}
% 	\end{subfigure}
% 	\caption{Real experiment results with 9 robots after 200 seconds of exploration.}
% 	\label{fig:real_ex_rez}
% \end{figure}

% This can be observed in Figure \ref{fig:perror_real}, which shows the localization RMSE for the SwarMap with and without the absolute localization sensor, as well as for odometry only estimation. Close to time $t=50$s, the error abruptly increases due to a collision that causes the average pose estimation to diverge. We can notice that the SwarMap using one GPS is capable of recovering from this error, as soon as the accurate information from the GPS robot is shared among the swarm. On the other hand, the other two approaches are not capable of reducing the localization error. Since the localization directly impacts the map quality, the maps generated by odometry only and by SwarMap without a GPS robot do not have a good quality in these real experiments.

% \begin{figure}
% %	\begin{subfigure}{.5\textwidth}
% 		\centering
% 		\includegraphics[width=0.94\columnwidth]{figures/rmse_reall_mac}
% 		%\caption{Position error}
% 		%label{fig:perror_real1}
% %	\end{subfigure}
% %	\begin{subfigure}{.5\textwidth}
% %		\centering
% %		\includegraphics[width=\linewidth]{figures/rmse_ang_real_mac.pdf}
% %		\caption{Orientation error}
% %		\label{fig:perror_real2}
% %	\end{subfigure}
% 	\caption{Average localization error for different approaches in experiments with real robots.}
% 	\label{fig:perror_real}
% \end{figure}
